Bounds on ALP-Mediated Dark Matter Models from Celestial Objects

We have studied the signals from axion-like particles (ALPs) as dark matter mediators from celestial objects such as neutron stars, brown dwarfs or white dwarfs. We consider the accumulation of dark matter inside the celestial objects using the multiscatter capturing process. The production of ALP from the dark matter annihilation can escape the celestial object and decay into gamma-rays and neutrinos before reaching the Earth. We investigate our model using gamma-ray observations from Fermi and H.E.S.S. and neutrino observations from IceCube and ANTARES. The effective Lagrangian approach allows us to place constraints on the ALP-photon and ALP-fermion couplings. In the gamma-ray channel, our results are able to rule out the existence of ALP with mass up to $\sim \mathcal{O}(10)$ GeV. On the other hand, the neutrino observations can be used to probe a higher mass range with ALP mass up to $\sim \mathcal{O}(100)$ GeV.

==> zbackup.tex <==

\newpage
\section{BACK UP}

\subsection{Model}

\begin{equation}
    \chi\bar{\chi} \rightarrow (inside) \rightarrow a \rightarrow (outside) \rightarrow\nu\bar{\nu}
\end{equation}
\textbf{Calculation $\chi f \rightarrow \chi f$}\\
\begin{center}

\begin{fmffile}{first-diagram}
 \begin{fmfgraph*}(100,100) %NOTE the fmfgraph* environment
   \fmfleft{i1,i2}
   \fmfright{o1,o2}
   \fmf{fermion,label=$f$}{i1,v1}
   \fmf{fermion,label=$f$}{v1,o1}
   \fmf{fermion,label=$\chi$}{i2,v2}
   \fmf{fermion,label=$\chi$}{v2,o2}
   \fmf{scalar,label=$a$}{v2,v1}
   % Add our labels
   \fmflabel{$g_{aff}$}{v1}
   \fmflabel{$g_{a\chi\chi}$}{v2}
 \end{fmfgraph*}
\end{fmffile}
\end{center}

\begin{eqnarray}
    -i\mathcal{M} = \left( \bar{u}_4^{r_2} g_{a\chi\chi}\textcolor{red}{(i)}\gamma^5 u_2^{s_2} \right)\frac{1}{p^2 - m_a^2} \left( \bar{u}_3^{r_1} g_{aff}\textcolor{red}{(i)}\gamma^5 u_1^{s_1} \right)
\end{eqnarray}
Compute the amplitude square
\begin{eqnarray}
    \sum_{\text{spin}}|\mathcal{M}|^2 & = &\frac{1}{(p^2 - m_a^2)^2}\left[ \left( \bar{u}_4^{r_2} g_{a\chi\chi}\textcolor{red}{(i)}\gamma^5 u_2^{s_2} \right)\left( \bar{u}_3^{r_1} g_{a\chi\chi}\textcolor{red}{(i)}\gamma^5 u_1^{s_1} \right)\right] \left[\left( \bar{u}_1^{s_1} g_{aff}\textcolor{red}{(-i)}\gamma^5 u_3^{r_1} \right)\left( \bar{u}_2^{s_2} g_{aff}\textcolor{red}{(-i)}\gamma^5 u_4^{r_2} \right)\right] \nonumber \\ 
    & = &\frac{g_{aff}^2g_{a\chi\chi}^2}{(p^2 - m_a^2)^2}\left[ ( \bar{u}_4^{r_2})^\alpha (\gamma^5)_\alpha^\beta (u_2^{s_2})_\beta  (\bar{u}_3^{r_1})^\rho  (\gamma^5)_\rho^\sigma (u_1^{s_1})_\sigma\right] \left[ (\bar{u}_1^{s_1})^\delta (\gamma^5)_\delta^\epsilon (u_3^{r_1})_\epsilon (\bar{u}_2^{s_2})^\lambda (\gamma^5)_\lambda^\kappa (u_4^{r_2})_\kappa \right] \nonumber \\
    & = &\frac{g_{aff}^2g_{a\chi\chi}^2}{(p^2 - m_a^2)^2} \left[ (\slashed{p}_4 + m_\chi)^\alpha_\sigma(\gamma^5)_\alpha^\beta(\slashed{p}_2 + m_\chi)^\rho_\beta(\gamma^5)_\rho^\sigma \right] \left[(\slashed{p}_3 + m_f)^\delta_\kappa(\gamma^5)_\delta^\epsilon(\slashed{p}_1 + m_f)^\lambda_\epsilon(\gamma^5)_\lambda^\kappa\right] \nonumber \\
    & = &\frac{g_{aff}^2g_{a\chi\chi}^2}{(p^2 - m_a^2)^2} (-4 g^{\mu\nu}p_{4,\mu}p_{2,\nu} + 4m^2_\chi)(-4 g^{\alpha\beta}p_{3,\alpha}p_{1,\beta} + 4m^2_f )
\end{eqnarray}
where $p = p_1 - p_3$. From $t=(p_1-p_3)^2=(p_4-p_2)^2$, therefore
\begin{equation}
    \sum_{\text{spin}}|\mathcal{M}|^2 = \frac{8 g_{aff}^2 g_{a\chi\chi}^2}{(t - m_a^2)^2} \left(\frac{t^2}{2} + m^4_\chi+ m^4_f + m^2_\chi m^2_f\right)
\end{equation}
We interested in the case of scattering in low-energy limit, i.e. $t\rightarrow 0$ and $s = (m_\chi + m_f)^2$. Therefore, we find
\begin{equation}
    \sum_{\text{spin}}|\mathcal{M}|^2 = \frac{8 g_{aff}^2 g_{a\chi\chi}^2}{m_a^4} \left(m^4_\chi+ m^4_f + m^2_\chi m^2_f\right).
\end{equation}
The cross-section in low-energy limit becomes
\begin{eqnarray}
    \sigma(\chi f \rightarrow \chi f) &=& \frac{1}{16\pi s}\sum_{\text{spin}}|\mathcal{M}|^2 \\
    &=& \frac{1}{16\pi (m_\chi + m_f)^2} \frac{8 g_{aff}^2 g_{a\chi\chi}^2}{m_a^4} \left(m^4_\chi+ m^4_f + m^2_\chi m^2_f\right) \nonumber \\
    \sigma(\chi f \rightarrow \chi f) &=& \frac{g_{aff}^2 g_{a\chi\chi}^2}{2\pi{m_a^4}} \frac{m^4_\chi+ m^4_f + m^2_\chi m^2_f}{(m_\chi + m_f)^2}. \label{eq:xsec}
\end{eqnarray}

\subsection{Decay width of $a\rightarrow ff$}

\begin{center}
\begin{fmffile}{complex-a}
 \begin{fmfgraph*}(100,100) %NOTE the fmfgraph* environment
   \fmfleft{i1}
   \fmfright{o1,o2}
   \fmf{fermion,label=$f_2$}{v1,o1}
   \fmf{fermion,label=$f_1$}{v1,o2}
   \fmf{scalar,label=$a$}{i1,v1}
   % Add our labels
   \fmflabel{$g_{aff}$}{v1}
 \end{fmfgraph*}
\end{fmffile}
\end{center}
\begin{eqnarray}
    \textcolor{red}{-i\mathcal{M} = \bar{v_1}ig_{aff}u_2}
\end{eqnarray}
\begin{eqnarray}
    \Gamma_{a\rightarrow ff} = \frac{g_{aff}^2n_f^c m_a}{8\pi}\sqrt{1-\frac{4m^2_f}{m_a^2}}
\end{eqnarray}
where $n_f^c$ is the number of colour degrees of freedom of the fermion.
 
\subsection{Decay width of $a\rightarrow \gamma\gamma$}

\begin{center}
\begin{fmffile}{complex-b}
 \begin{fmfgraph*}(100,100) %NOTE the fmfgraph* environment
   \fmfleft{i1}
   \fmfright{o1,o2}
   \fmf{photon,label=$\gamma$}{v1,o1}
   \fmf{photon,label=$\gamma$}{v1,o2}
   \fmf{scalar,label=$a$}{i1,v1}
   % Add our labels
   \fmflabel{$g_{a\gamma\gamma}$}{v1}
 \end{fmfgraph*}
\end{fmffile}
\end{center}
Note that $g_{aff}$ is effective coupling.
\begin{eqnarray}
    -i\mathcal{M} & = & \epsilon_\mu(p_1)ig_{a\gamma\gamma}\epsilon^*_\nu(p_2) \\
    & = & \textcolor{red}{i g_{a\gamma\gamma}k_\sigma p_\rho \epsilon^{\mu\nu\rho\sigma} \epsilon_\mu(p) \epsilon_\nu(k).}
\end{eqnarray}
\begin{eqnarray}
    %\Gamma_{a\rightarrow \gamma\gamma} = 4 g_{aff}^2
    \Gamma_{a\rightarrow \gamma\gamma} = \frac{1}{4\pi}\frac{g_{a\gamma\gamma}^2}{m_a} \textcolor{red}{=\frac{1}{64\pi}g^2_{a\gamma\gamma}m_a^3}
\end{eqnarray}

\subsection{Dark matter capturing}

It's not spin dependent as in the gauge boson mediators, so we might have to carefully check the possibility of capturing dark matter using axion mediator.

%\subsection{Details of calculations}
From ref \cite{Bramante:2017xlb} and \cite{Dasgupta:2019juq} and \cite{Chen:2023fgr}. \\

In order to study the multiple scatter capturing of dark matter, let's consider the single scattering case. Consider the following conditions

From far away from the stars, the speed of dark matter follow Boltzmann distribution. Half of DM particles will be moving towards to the star with $ - \pi/2 < \theta < \pi/2$, where $\theta$ is the angle between the velocity of DM particles and a vector that pointing to the center of the star. The total DM flux is defined as $\mathcal{F}$. The gravitational potential of the star will cause DM to move faster as they approach it, but the conservation of momentum implies that the angular momentum with respect to the star must be fixed. Therefore we can determine that whether the angular momentum of the particle is small enough to intersect a spherical mass shell at radius $r$ by knowing $\theta$ and initial speed of particle. The probability that DM scatters and is captured while it transits a mass shell of thickness $dr$ depends on the density of scattering sites $n(r)$, the initial velocity of DM $\vec{u}$ and the cross-section of DM with stellar constituents $\sigma$. To determine the total capture rate, we integrate the Boltzmann distribution for capture over $0< u < \infty$ for each stellar mass shell, and integrate mass shell over $0<r<R$.

We assume that the velocity of dark matter follows a Maxwell-Boltzmann distribution. The number density of dark matter with velocity from $u$ to $u+du$ is
\begin{equation}
    f(u)du = 3\sqrt{\frac{6}{u}}\frac{n_X u^2}{\bar{v}^3} \text{exp}\left( -\frac{3}{2}\frac{u^2}{\bar{v}^2} \right), \label{eq:fdu}
\end{equation}
where $n_X$ is the number density of dark matter and $\bar{v}$ is the average velocity. The above equation gives the distribution of the velocity of dark matter far from the gravitational well. The total velocity of dark matter close to the star is given by $w^2 = u^2 + v^2(r)$, where $v(r)$ is the escape velocity at radius $r$.

Consider the flux of DM across the large sphere that the gravitational potential of the star can be neglected. In this case, the angle at DM intersect the large sphere can affect the its flux across the surface, therefore, the factor of $\vec{u}\cdot\hat{R_a} = u \cos\theta$ must taking into account, where $\theta$ is the angle between the DM's velocity $\vec{u}$ and a unit vector that normal to the large surface $\hat{R_a}$. The flux of dark matter flux is obtained by integrating the product of $u\cos\theta$ and equation \ref{eq:fdu} over $0<d(\cos\theta)<1$. The factor of 1/2 is also included in order to reject the out going particles, we have
\begin{equation}
    dF = \frac{1}{2}f(u)u \cos\theta\ du\ d(\cos\theta) = \frac{1}{4} f(u) u \ du \ d(\cos^2\theta). 
\end{equation}
This leads to the flux of dark matter entering the shpere of size $R_a$,
\begin{equation}
    d\mathcal{F} = 4\pi R_a^2 dF = \pi R_a^2  f(u) u \ du \ d(\cos^2\theta). \label{eq:fluxentering}
\end{equation}
In order to obtained the capture rate, we must consider the dark matter flux will inside the spherical shell at radius $r$. The dimensonless angular momentum of dark matter is
\begin{equation}
    J \equiv u R_a \sin \theta = w r \sin \alpha, \label{eq:angmomentum}
\end{equation}
where $\alpha$ is the angle between the dark matter's velocity $\vec{w}$ and the unit vector normal to the shperical shell $\hat{r}$. The dark matter flux, equation \ref{eq:fluxentering} can be rewrite with $dJ^2 = u^2 R_a^2 d(\cos^2\theta)$ as 
\begin{equation}
    d\mathcal{F} = \pi f(u)\frac{du}{u} dJ^2. \label{eq:dF}
\end{equation}

The probability of dark matter being captured after scattering once defined as $g_1(w)$. The total probability of capturing dark matter is
\begin{equation}
     n(r)\sigma g_1(w) dl, \label{eq:n}
\end{equation}
where $n(r)$ indicates the number density of scattering sites and $dl = dr/\cos\alpha$ is length in spherical shell. Using the equation \ref{eq:angmomentum}, we can rewrite $dl$ as
\begin{equation}
    dl = dr / \sqrt{1 - (J/rw)^2}.
\end{equation}
The total single scatter capture rate can be obtained by multiplying equations \ref{eq:dF} and \ref{eq:n} and integrate over $J$. To make sure that the angular momentum of dark matter is small enough to intersect a shell of size $r$, the theta function $\Theta(rw - J)$ is applied. The factor of two is multiplied in order to account the dark matter passing both side. Therefore, the scatter capture rate is
\begin{eqnarray}
    dC_1 &=& 2 \int_0^\infty \ \pi f(u)\frac{du}{u} dJ^2 \ n(r)\sigma g_1(w)dl \ \Theta(rw - J)\\
    &=&  2\pi \sigma n(r) g_1(w) f(u)\frac{du}{u} \int_0^\infty \Theta(rw - J)\ dl dJ^2 \\
    &=&  2\pi \sigma n(r) g_1(w) f(u)\frac{du}{u} \int_0^\infty \Theta(rw - J)\ \left( \frac{dr}{ \sqrt{1 - (J/rw)^2}}\right) (2J \ dJ) \\
    &=& 4\pi \sigma n(r) g_1(w) f(u)\frac{du}{u} w^2r^2\ dr. \label{eq:dc}
\end{eqnarray}




The fraction energy loss of single elastic scattering dictate is distributed in the range 
\begin{equation}
    0 \leq \frac{\Delta E}{E_0} \leq \beta_+,
\end{equation}
where 
\begin{equation}
    \beta_\pm \equiv \frac{4 m_\chi m_f}{(m_\chi \pm m_f)^2},
\end{equation}
where $m_\chi$ is DM mass and $m_f$ is the target mass. The fraction of kinetic energy loss for capturing is $u^2/w^2$ which is the ratio of the kinetic energy of DM from far away versus inside the star. To find $g_1(w)$ we use the probability for a single scatter
\begin{equation}
    \frac{1}{\beta_+}\left( \beta_+ - \frac{u^2}{w^2} \right), \label{eq:facE}
\end{equation}
and a step function to unsure the dark matter is captured after a single scatter
\begin{equation}
    \Theta\left( \beta_+ - \frac{u^2}{w^2} \right) .\label{eq:Theta}
\end{equation}
The probability $g_1(w)$ is obtained by multiply equation \ref{eq:facE} and \ref{eq:Theta}, the results is
\begin{eqnarray}
    g_1(w) = \frac{1}{\beta_+}\left( \beta_+ - \frac{u^2}{w^2} \right)\Theta\left( \beta_+ - \frac{u^2}{w^2} \right)
\end{eqnarray}

Integrate over the incoming Boltzmann distribution to find the total capture rate of single scatter as a function of radius
\begin{eqnarray}
    C_1 = \pi\sqrt{\frac{96}{\pi}}\frac{n_X}{\bar{v}}\int^R_0 dr\  r^2 n(r)\sigma(r)v^2(r) \left( 1 - \frac{1 - e^{-A^2(r)}}{A^2(r)} \right),
\end{eqnarray}
where $A^2 \equiv 3v^2(r)/2\bar{v}^2\beta_- $. In limit of $v(r) \sim v_{esc}(R)$, the single capture rate is
\begin{eqnarray}
    C_1 = \sqrt{24\pi}G \frac{\rho_X}{m_X} MR \frac{1}{\bar{v}} \text{Min}\left[ 1, \frac{\sigma}{\sigma_{sat}}\right]\left( 1 - \frac{1 - e^{-A^2}}{A^2} \right).
\end{eqnarray}

Now let's evaluate the capture rate of the case of multiplescatter. Consider the case of $N$ scatter, the probability of DM with optical dept $\tau$ is described by
\begin{eqnarray}
    p_N(\tau) = 2 \int_0^1 dy \frac{y e^{-y\tau} (y\tau)^N}{N!}.
\end{eqnarray}
The optical dept is defined as $\tau = 3\sigma/2\sigma_{sat}$, where $\sigma$ is the cross-section of DM with nucleon, and $\sigma_{sat} = \pi R^2/N_n$ where $N_n$ is the number of scattering sites per star. If the number of interactions exceeds $N\sim n\sigma R( \textcolor{red}{n\sigma (2R))}$, DM will be slowed by multiple scatters. The differential of DM capture rate after N scatter is looks similar to the case of single scatter. From equation \ref{eq:dc}, we find
\begin{eqnarray}
    C_N = \pi R^2 p_N(\tau) \int_0^\infty f(u)\frac{du}{u} w^2 g_N(w).
\end{eqnarray}
or
\begin{eqnarray}
    C_N = \pi R^2 p_N(\tau) \int_{\nu_e}^\infty dw \frac{f(u)}{u^2} w^3 g_N(w). \label{eq:c_n_int}
\end{eqnarray}
Total capture rate is the sum over all $N$, therefore
\begin{eqnarray}
    C_{tot} = \sum_{N=1}^\infty C_N.
\end{eqnarray}

Let's consider the probability $g_N(w)$. The probability after $N$ scatter should depend on dark matter’s initial velocity, the amount of energy lost in each scatter, and the escape velocity of the star. The initial kinetic energy of DM at star surface is $E_0 = m_X w^2/2$, the kinetic lost after single scatter is $\delta E = z\beta_+ E_0$, where $z$ is related to scattering angle $z\supset [0,1]$ and $ \beta_+ \equiv {4 m_\chi m_f}/{(m_\chi + m_f)^2}$. The DM's kinetic energy and velocity after $N$ scattering are
\begin{eqnarray}
    E_N = \prod_{i=1}^N\left( 1 - z_i \beta_+ \right)E_0, \quad v_N = \prod_{i=1}^N\left( 1 - z_i \beta_+ \right)^{1/2}w.
\end{eqnarray}

If the velocity after $N$ scatter is less than the escape velocity, DM is captured. From the initial velocity $w$, the capture probability is
\begin{eqnarray}
    g_N(w) = \int_0^1 dz_1 \int_0^1 dz_2 \int_0^1 dz_3 \ldots \int_0^1 dz_N \Theta( v_{esc}\prod_{i=1}^N\left( 1 - z_i \beta_+ \right)^{1/2} - w ),
\end{eqnarray}
where $dz_i$ sums over all possible trajectories at each step. We replace $z_i$ with their average value, $g_N(w)$ can simplifies as
\begin{eqnarray}
    g_N(w) \approx \Theta\left( v_{esc}(1 - \langle z_i\rangle\beta_+)^{-N/2} \right).
\end{eqnarray}
From equation \ref{eq:c_n_int}, after apply $g_N(w)$, we obtain the multiscatter capture rate as
\begin{eqnarray}
    C_N = \pi R^2 p_N(\tau) \frac{\sqrt{6}n_X}{3\sqrt{\pi}\bar{v}}\left( (2\bar{v}^2 + 3v^2_{esc}) - (2\bar{v}^2 + 3v^2_N) \text{exp}\left( - \frac{3}{2}\frac{(2v_N^2 + 3v^2_{esc}) }{\bar{v}^2} \right)  \right). %\label{eq:capturerate}
\end{eqnarray}
